Learning the Depths of Moving People by Watching Frozen People

We present a method for predicting dense depth in scenarios where both a monocular camera and people in the scene are freely moving. Existing methods for recovering depth for dynamic, non-rigid objects from monocular video impose strong assumptions on the objects' motion and may only recover sparse depth. In this paper, we take a data-driven approach and learn human depth priors from a new source of data: thousands of Internet videos of people imitating mannequins, i.e., freezing in diverse, natural poses, while a hand-held camera tours the scene. Because people are stationary, training data can be generated using multi-view stereo reconstruction. At inference time, our method uses motion parallax cues from the static areas of the scenes to guide the depth prediction. We demonstrate our method on real-world sequences of complex human actions captured by a moving hand-held camera, show improvement over state-of-the-art monocular depth prediction methods, and show various 3D effects produced using our predicted depth.

==> implementation.tex <==
\subsection{Losses}
Because depth values produced by our data pipeline have arbitrary scale, we use a scale-invariant depth regression loss. That is, our loss is computed on log-space depth values and consists of three terms:
\begin{align}
  \Lsi = \Lmse + \alpha_1 \Lgrad + \alpha_2 (\Lsmf + \Lsms). \label{eq:Loss}
\end{align}
\noindent \textbf{Scale-invariant MSE.}  We evaluate the mean square error (MSE) of the difference between all pairs of log-depths to achieve scale invariance~\cite{eigen2014depth}:
{\small \begin{align}
    \Lmse = \frac{1}{N} \sum_{\mathbf{p}} (R(\mathbf{p}))^2  -  \frac{1}{N} \left( \sum_{\mathbf{p}} R(\mathbf{p}) \right)^2, 
\end{align}}
where  $R(\mathbf{p}) = \log \hat{D}(\mathbf{p}) - \log \DMVS (\mathbf{p})$;   $\hat{D}$ is the predicted depth and $\DMVS$ is the ground truth MVS depth. 

\smallskip
\noindent \textbf{Multi-scale gradient matching term.}
We use a multi-scale gradient matching term to encourage smoother gradient changes and sharper depth discontinuities in the predicted depth images~\cite{li2018megadepth}:
{\small
\begin{align}
  \Lgrad & = \sum_{s=0}^{S-1} \frac{1}{N_s} \sum_{\mathbf{p}} \left( \left|\nabla_x R_s(\mathbf{p}) \right|
  + \left| \nabla_y R_s(\mathbf{p}) \right| \right) 
  \label{eq:loss_grad}
\end{align}}
where subscript $s$ of $R_s$ indicates scale $s$ and $N_s$ is the number of valid pixel at scale $s$. 

\medskip
\noindent \textbf{Multi-scale, edge-aware smoothness terms.}
To encourage smooth interpolation of depth in texture-less regions where MVS fails to recover depth, we add a simple smoothness term at multiple scales based on the first- and second-order statistics of images~\cite{Wang_2018_CVPR}:
{\small
\begin{align}
    \Lsmf & = \sum_{s=0}^{S-1} \frac{1}{N_s 2^{s}} \sum_{\mathbf{p}}\exp(- |\nabla I_s(\mathbf{p})| ) | \nabla \log \hat{D}(\mathbf{p}) | \\
    \Lsms & = \sum_{s=0}^S \frac{1}{N_s 2^{s}} \sum_{\mathbf{p}} \exp(- |\nabla^2 I_s(\mathbf{p})|) | \nabla^2 \log \hat{D}(\mathbf{p}) |
\end{align}}
We create $S=5$ scale image pyramids using nearest-neighbor down-sampling for both gradient matching and smoothness terms. 



==> intro_backup.tex <==
\section{Introduction}

A hand-held camera viewing a dynamic scene is a common scenario in modern photography. Recovering dense geometry in this case is a challenging task: 
moving objects violate the epipolar constraint used in 3D vision, and are often treated as noise or outliers in existing Structure-from-Motion (SfM) and Multi-view Stereo (MVS) methods. %
Our human depth perception, however, is not easily fooled by object motion--rather, we maintain a feasible interpretation of the objects' geometry and depth ordering even when both the observer and the objects are moving, and even when the scene is observed with just one eye~\cite{howard2002seeing}. In this work, we take a step towards achieving this ability computationally. 
\footnotetext{In all figures, we use inverse depth maps for visualization purposes, and refer to them as depth maps.}

We focus on the task of predicting accurate, dense depth from ordinary videos where both the camera and  \emph{people} in the scene are \emph{naturally moving}. We focus on humans for two reasons: (i) human motion is typically articulated and non-rigid, thus difficult to explicitly model, and (ii) in many applications such as augmented reality (AR), humans constitute the salient objects the scene. We take advantage of the video input by focusing on the two-view case, where we observe a dynamic scene from two different viewpoints at different times. This allows us to benefit from information  beyond single view. 

We design and train a deep neural network that takes an input RGB image, a human mask, and an initial environmental depth estimated from two frames (see Fig.~\ref{fig:teaser}), and outputs a dense depth map over the \emph{entire} image, both the environment and the people. By taking a data-driven approach, we avoid the need to explicitly impose assumptions on the deformation or shape configuration of the people, but rather learn these priors from the data.



Where do we get data to train such a method? Generating high-quality synthetic data in which both the camera and the people in the scene are naturally moving is very challenging.
RGBD sensors such as Kinect can provide useful data, but such depth sensors are typically limited to indoor environments and require significant manual work in capturing and synchronization. Moreover, it is difficult to gather people of different ages, genders with diverse poses at scale. Instead, we derive data from a surprising source: YouTube videos
in which people imitate mannequins, i.e., freeze in elaborate, natural poses, while a hand-held camera tours the scene (Fig.~\ref{fig:dataset}). These type of videos comprise our new \emph{\Dataset (\DatasetShort)} dataset, which we plan to release for the research community. Since the entire scene, including the people, is stationary, we infer the camera poses and estimate depth using SfM and MVS, which serves as supervision for training.

We demonstrate the applicability of our method in the real-world scenario of Internet video shot with a hand-held camera, depicting complex human actions such as walking, running, and dancing. Our approach estimates depth to higher accuracy 
than state-of-the-art monocular depth prediction and motion stereo methods. Our depth maps can also be used to produce various 3D effects including depth re-focusing, 
depth inpainting, and inserting virtual objects into the 3D scene with correct occlusion. 

In summary, our contributions are: (i) a new source of data  for depth prediction consisting of a large number of Internet videos in which the camera moves around people ``frozen'' in natural poses, along with a methodology for generating accurate depth maps and camera poses; (ii) a deep-network-based model designed and trained to predict dense depth maps in the challenging case of simultaneous camera motion and complex human motion. We hope these principles and data will aid new research in monocular, dynamic scene reconstruction.



